InternVL: Scaling up Vision Foundation Models and Aligning for Generic Visual-Linguistic Tasks

The exponential growth of large language models (LLMs) has opened up numerous possibilities for multimodal AGI systems. However, the progress in vision and vision-language foundation models, which are also critical elements of multi-modal AGI, has not kept pace with LLMs. In this work, we design a large-scale vision-language foundation model (InternVL), which scales up the vision foundation model to 6 billion parameters and progressively aligns it with the LLM, using web-scale image-text data from various sources. This model can be broadly applied to and achieve state-of-the-art performance on 32 generic visual-linguistic benchmarks including visual perception tasks such as image-level or pixel-level recognition, vision-language tasks such as zero-shot image/video classification, zero-shot image/video-text retrieval, and link with LLMs to create multi-modal dialogue systems. It has powerful visual capabilities and can be a good alternative to the ViT-22B. We hope that our research could contribute to the development of multi-modal large models. Code and models are available at https://github.com/OpenGVLab/InternVL.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/dataset.tex <==
\begin{table}[ht]\scriptsize
    \centering
    \begin{subtable}{0.53\linewidth}  % 创建第一个子表格，占据页面宽度的一半
        \centering
        \setlength\tabcolsep{1pt}
        \renewcommand{\arraystretch}{1.05}
      \begin{tabular}{l|cccccc|c|c}
        method &  IN-1K &  IN-A &  IN-R &  IN-V2 &  IN-Ske &  ObjectNet & $\Delta${$\downarrow$} & avg. \\
        \hline

         OpenCLIP-H &
         78.0 &  59.3 &  89.3 &  70.9 &  66.6 &  69.7 & 5.7 &  72.3\\
         
         OpenCLIP-g & 
         78.5 &  60.8 &  90.2 &  71.7 &  67.5 &  69.2 & 5.5 &  73.0 \\
         
         OpenAI CLIP-L+ &
         76.6 &  77.5 &  89.0 &  70.9 &  61.0 &  72.0 & 2.1 &  74.5 \\
         
         EVA-01-CLIP-g &
         78.5 &  73.6 &  92.5 &  71.5 &  67.3 &  72.3 & 2.5 &  76.0 \\
         
         OpenCLIP-G & 
         80.1 &  69.3 &  92.1 &  73.6 &  68.9 &  73.0 & 3.9 &  76.2\\
         
         EVA-01-CLIP-g+ & 
         79.3 &  74.1 &  92.5 &  72.1 &  68.1 &  75.3 & 2.4 &  76.9\\
         
         EVA-02-CLIP-L+ &
         80.4 &  82.9 &  93.2 &  73.8 &  68.9 &  78.4 &  \textbf{0.8} &  79.6 \\
         
         EVA-02-CLIP-E &
         81.9 &  80.4 &  94.1 &  75.4 &  71.8 &  76.9 &  1.8 &  80.1\\
         
         EVA-02-CLIP-E+ & 
         82.0 &  82.1 &  94.5 &  75.7 &  71.6 &  79.6 &  1.1 &  80.9\\

         \textcolor{gray}{CoCa$^\dagger$} & 
         \textcolor{gray}{86.3} &  \textcolor{gray}{90.2} &  \textcolor{gray}{96.5} &  \textcolor{gray}{80.7} &  \textcolor{gray}{77.6} &  \textcolor{gray}{82.7} & \textcolor{gray}{0.6}  &  \textcolor{gray}{85.7} \\

        \hline
         \rowcolor{gray!20}
         InternVL-CLIP &
         \textbf{83.2} &	\textbf{83.8} &	\textbf{95.5} &	\textbf{77.3} &	\textbf{73.9} &	\textbf{80.6} &	\textbf{0.8} &  \textbf{82.4} \\
    \end{tabular}
        \caption{ImageNet variants and ObjectNet.}
        \label{subtable:a}
    \end{subtable}%
    \vspace{0.5em}
    \begin{subtable}{0.46\linewidth}  % 创建第一个子表格，占据页面宽度的一半
        \centering
        \setlength\tabcolsep{3pt}
        \renewcommand{\arraystretch}{1.05}
      \begin{tabular}{l|ccccc|c}
        method &  EN &  ZH &  JP &  AR &  IT &  avg. \\

        \hline
        CLIP-Italian  &
        $-$	& $-$ & $-$ & $-$ & 22.1 & $-$ \\

        Japanese-CLIP-ViT-B &
        $-$	& $-$ & 54.6 & $-$ & $-$ & $-$ \\
        
        Taiyi-CLIP-ViT-H &
        $-$	& 54.4 & $-$ & $-$ & $-$ & $-$ \\

        WuKong-ViT-L-G &
        $-$	& 57.5 & $-$ & $-$ & $-$ & $-$ \\

        WuKong-Swin-L &
        $-$	& 58.2 & $-$ & $-$ & $-$ & $-$ \\
        
        CN-CLIP-ViT-H &
        $-$	& 59.6 & $-$ & $-$ & $-$ & $-$ \\

        AltCLIP-ViT-L &
        74.5 & 59.6 & $-$ & $-$ & $-$ & $-$ \\

        EVA-02-CLIP-E+ & 
        82.0 & 3.6 & 5.0 & 0.2 & 41.2 & 26.4 \\

        % \hline
        
        OpenCLIP-XLM-R-B &
        62.3 &	42.7 &	37.9 &	26.5 &	43.7 &	42.6  \\

        OpenCLIP-XLM-R-H &
        77.0 &	55.7 &	53.1 &	37.0 &	56.8 &	55.9  \\
        
        \hline
         \rowcolor{gray!20}
         InternVL-CLIP &
         \textbf{83.2} &	\textbf{64.5} &	\textbf{61.5} &	\textbf{44.9} &	\textbf{65.7} &	\textbf{64.0}  \\
    \end{tabular}
        \caption{Multilingual ImageNet-1K.}
        \label{subtable:a}
    \end{subtable}%
    \vspace{-0.5em}
    \caption{\textbf{Comparison of zero-shot image classification performance.} 
    ``{$\Delta$\scriptsize$\downarrow$}'': The gap between the averaged top-1 accuracy and the IN-1K top-1 accuracy. 
    $^\dagger$ CoCa~\citep{yu2022coca} uses the JFT-3B dataset~\citep{zhai2022scaling} with label names for pretraining.
    Multilingual evaluation involves 5 languages, including English (EN), Chinese (ZH), Japanese (JP), Arabic (AR), and Italian (IT).
    }
    \vspace{-0.5em}
    \label{table:main}
\end{table}


==> table/zero-shot-vqa.tex <==
\begin{table*}[t]\scriptsize
\renewcommand{\arraystretch}{1.0}
\begin{subtable}{1\textwidth}
    \centering
    \setlength\tabcolsep{6pt}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
        & \multicolumn{3}{c|}{Image Captioning} & \multicolumn{7}{c}{Visual Question Answering} \\
        & COCO & Flickr30k & NoCap & VQAv2 & OKVQA & VizWiz &  GQA  & VisDial  & TextVQA & SciQA  \\
        method & karpathy test & karpathy test     &  val  & test-dev &  test  & test-dev & test-dev & val & test &  \\
        \hline
        
        % MetaLM~\cite{hao2022metavlm} & 
        % 82.2 & 43.3 & 58.7 & 41.1 & 11.4 & $-$ & $-$ & $-$ & $-$ & $-$ \\
        
        Flamingo-9B~\cite{alayrac2022flamingo} & 
        79.4 & 61.5 & $-$ & 51.8 & 44.7 & 28.8 & $-$ & 48.0 & 31.8 & $-$ \\
        
        Flamingo-80B~\cite{alayrac2022flamingo} & 
        84.3 & 67.2 & $-$ & 56.3/82.0$^*$ & 50.6 & 31.6 & $-$ & 52.0 & 35.0 & $-$ \\
        
        SimVLM~\cite{wang2021simvlm} & 
        143.3$^*$  & $-$  & 112.2 & 80.0$^*$  & $-$  & $-$  & $-$  & $-$ & $-$ & $-$ \\
        
        CoCa~\cite{yu2022coca} &
        143.6$^*$  & $-$  & 122.4 & 82.3$^*$  & $-$  & $-$  & $-$  & $-$ & $-$ & $-$ \\
        
        BLIP~\cite{li2022blip} & 
        136.7$^*$  & $-$  & 113.2 & 78.3$^*$  & $-$  & $-$  & $-$  & 69.4$^*$  & $-$ & $-$ \\
        
        BLIP-2~\cite{li2023blip2} & 
        144.5$^*$  & $-$  & 121.6 & 65.0/82.2$^*$ & 45.9 & $-$  & 44.7 & $-$ & 42.4 & $-$ \\

        InstructBLIP (Vicuna-7B)~\cite{instructblip} & 
        $-$  & 82.4 & 123.1 & $-$  & $-$  & 34.5 & 49.5  & 48.5 & 50.7 & \\
        
        InstructBLIP (Vicuna-13B)~\cite{instructblip} & 
        $-$  & 82.8 & 121.9 & $-$  & $-$  & 34.5 & 49.5  & 48.5 & 50.7 & \\
        
        Shikra-13B (Vicuna-13B)~\cite{chen2023shikra} &
        117.5$^*$  & 73.9 &  $-$  & 77.4$^*$  & 47.2 & $-$  & $-$  & $-$ & $-$ & $-$\\
        
        KOSMOS-1~\cite{huang2023kosmos1} & 
        84.7 & 67.1 &  $-$  & 51.0 & $-$  & 29.2 & $-$  & $-$ \\
        
        KOSMOS-2~\cite{peng2023kosmos2} & 
        $-$  & 66.7 &  $-$  & 45.6 & $-$  & $-$  & $-$  & $-$ \\
        
        % ASM~\cite{wang2023allseeing} & $-$  & 87.7 & 117.2 & $-$  & $-$  & $-$  & $-$  & $-$ \\
        
        Emu~\cite{sun2023emu} & 
        112.4 & $-$ &  $-$  & 52.0 & 38.2 & 34.2 & $-$  & 47.4 & $-$ \\
        
        Emu-I~\cite{sun2023emu} & 
        117.7 & $-$ &  $-$  & 40.0 & 34.7 & 35.4 & $-$  & 48.0 & $-$ \\
        
        DreamLLM~\cite{dong2023dreamllm} & 
        115.4 & $-$ &  $-$  & 56.6 & 44.3 & 38.1 & $-$  & $-$ & 34.9 \\
        
        Qwen-VL~\cite{bai2023qwen} & 
        $-$ & 85.8 & 121.4 & 79.5$^*$ & 58.6$^*$ & 35.2 & 59.3$^*$ & $-$ & 63.8 & 67.1 \\
        
        Qwen-VL-Chat~\cite{bai2023qwen} &
        $-$ & 81.0 & 120.2 & 78.2$^*$ & 56.6$^*$ & 38.9 & 57.5$^*$ & $-$ & 61.5 & 68.2 \\
        
        LLaVA-1.5 \\
        
        \rowcolor{gray!15}
        InternVL-QLLaMA &
        \textbf{128.2} & 79.2 & 113.7 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\  

        \rowcolor{gray!15}
        InternVL-Chat &
        &  &  &  &  &  &  &  &  &  \\  
        
         
    \end{tabular}
\end{subtable}
\caption{\textbf{Comparison of image captioning and visual question answering.}
$^\dagger$These models are finetuned with the COCO dataset and zero-shot transferred to other datasets.
}
\label{tab: zs_cap_vqa}
\end{table*}
